Neutrino Mass Hierarchy

The neutrino mass hierarchy, i.e., whether the $\nu_3$ neutrino mass eigenstate is heavier or lighter than the $\nu_1$ and $\nu_2$ mass eigenstates, is one of the remaining undetermined fundamental features of the neutrino Standard Model. Its determination would represent an important step in the formulation of the generalized model, and would have a profound impact on the quest of the nature of neutrinos (Dirac or Majorana) and the search for a theory of flavor. In this review, we summarize the status of experimental and theoretical work in this field and explore the future opportunities that emerge in light of the recently discovered non-zero and relatively large third neutrino mixing angle $\theta_{13}$.

==> MH_stat.tex <==
\section{Statistical Issue in the Mass Hierarchy Determination}



\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics*[width=0.45\textwidth]{./figures/gaus_DT11}
&
\includegraphics*[width=0.45\textwidth]{./figures/MH_stat_prob}
\end{tabular}
\end{center}
\caption{\label{fig:mh:stat}  (left panel) The $T$ probability
distribution function for JUNO with \protect{$\Delta \chi^2_{\rm MH}
\approx 11$}, and (right panel) several sensitivity metrics in the
Bayesian statistics with resect to \protect{$\overline{\Delta T}\approx
\Delta\chi^2_{\rm MH}$}.}
\end{figure}

==> Makefile <==
##########################################################################
#
# $Id: Makefile,v 1.2 2010/10/29 15:06:33 slavic Exp $
#
##########################################################################
TEX = pdflatex
BIB = bibtex
DVIPDF = dvips
#main file
texfile = MH_review
#all figures
FIGS=$(wildcard figures/*.*)
#all texfiles
SECS=$(wildcard ./*.tex)
#SECS=$(wildcard sections/*.tex)

#export TEXINPUTS:=$(CURDIR):$(CURDIR)/elsstyle:$(TEXINPUTS)
#export BSTINPUTS:=$(CURDIR):$(CURDIR)/elsstyle:$(BSTINPUTS)
#export BIBINPUTS:=$(CURDIR):$(CURDIR)/elsstyle:$(BIBINPUTS)

.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

$(texfile).pdf : $(SECS) $(texfile).tex $(texfile).bib #$(FIGS) 
	$(TEX) $(texfile)
	$(BIB) $(texfile) # compile bibliography
	$(TEX) $(texfile)
	$(TEX) $(texfile)
	#$(DVIPDF) $(texfile).dvi
clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}

